RangeLDM: Fast Realistic LiDAR Point Cloud Generation

Autonomous driving demands high-quality LiDAR data, yet the cost of physical LiDAR sensors presents a significant scaling-up challenge. While recent efforts have explored deep generative models to address this issue, they often consume substantial computational resources with slow generation speeds while suffering from a lack of realism. To address these limitations, we introduce RangeLDM, a novel approach for rapidly generating high-quality range-view LiDAR point clouds via latent diffusion models. We achieve this by correcting range-view data distribution for accurate projection from point clouds to range images via Hough voting, which has a critical impact on generative learning. We then compress the range images into a latent space with a variational autoencoder, and leverage a diffusion model to enhance expressivity. Additionally, we instruct the model to preserve 3D structural fidelity by devising a range-guided discriminator. Experimental results on KITTI-360 and nuScenes datasets demonstrate both the robust expressiveness and fast speed of our LiDAR point cloud generation.

==> tables/DM_rebuttal.tex <==
\begin{table}[t]
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|ccc}
\hline
 Model & Model Size (M) & $\text{MMD}_\text{BEV}$ $\downarrow$ & $\text{FRD}_\text{range}$ $\downarrow$ & $\text{JSD}_\text{BEV}$ $\downarrow$ \\
\hline
 Ours & 41.4 & $\mathbf{3.07 \times 10^{-5}}$ & 1074.9 & 0.045  \\ 
\hline
 Ours-DM & 114.7  & $4.14 \times 10^{-5}$ & $\mathbf{899.0}$ & $\mathbf{0.040}$  \\ 
 Ours-DMS & 40.3 & $5.90\times 10^{-4}$ & $1889.3$ & $0.090$ \\ 
\hline
\end{tabular}
} 
\caption{Performance of different variants. ``Ours-DMS" is an ``Ours-DM" variant with a model size similar to ``Ours".}
\label{tab:DM_rebuttal}
\end{table}

==> tables/ablation_old.tex <==
\begin{table}[t]
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ccc|cccc}
\hline
 \makecell{Hough \\ Voting} & \makecell{Direction \\ Conditioned} & VAE & $\text{MMD}_\text{BEV}$ $\downarrow$ & $\text{FRD}_\text{range}$ $\downarrow$ & $\text{JSD}_\text{BEV}$ $\downarrow$ & \makecell{Throughput $\uparrow$ \\ (samples/s)}\\
\hline
 $\checkmark$   & $\times$  & $\checkmark$     &  $3.90 \times 10^{-4}$ & 1797.2	& 0.078  & -\\ 
 $\times$ &     $\checkmark$ & $\checkmark$    & $3.58 \times 10^{-4}$ & 1393.3 & 0.068 & -\\
 $\checkmark$ & $\checkmark$ & $\times$   & $4.14 \times 10^{-5}$ & $\mathbf{899.0}$ & $\mathbf{0.040}$ & 0.64 \\ 
 $\checkmark$ & $\checkmark$   & $\checkmark$ & $\mathbf{3.07 \times 10^{-5}}$ & 1074.9 & 0.045 & $\mathbf{4.86}$ \\ 
\hline
\end{tabular}
} 
\caption{Main ablation study. }
\label{tab:ablation}
\end{table}

==> tables/ablation_rebuttal.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
model & \makecell{Circular \\ Convolution} & \makecell{Direction \\ Conditioned} & \makecell{Hough \\ Voting}  &  $\text{MMD}_\text{BEV}$ $\downarrow$ & $\text{FRD}_\text{range}$ $\downarrow$ & $\text{JSD}_\text{BEV}$ $\downarrow$ \\
\hline
1 & $\times$     & $\times$      & $\times$     & $3.95 \times 10^{-4}$  & $1536.7$	& $0.067$  \\ 
2 & $\times$     & $\times$      & $\checkmark$     & $4.72\times 10^{-5}$  & $1103.1$	& $0.051$  \\ 
 \hline
 % $\times$       & $\times$  & $\checkmark$     &  $5.56 \times 10^{-4}$ & 1933.7	& 0.086  \\ 
3 & $\checkmark$   & $\times$  & $\times$     & $5.58 \times 10^{-4}$  & $1847.5$	& $0.179$  \\ 
 % $\checkmark$   & $\times$  & $\checkmark$     &  $3.90 \times 10^{-4}$ & 1797.2	& 0.078  \\ 
4 & $\checkmark$ & $\checkmark$   & $\times$ & $3.58 \times 10^{-4}$ & 1393.3 & 0.068 \\
5 & $\checkmark$ & $\checkmark$   & $\checkmark$ & $\mathbf{3.07 \times 10^{-5}}$ & $\mathbf{1074.9}$ & $\mathbf{0.045}$  \\ 
\hline
\end{tabular}
} 
\caption{Ablation study that involves circular convolution. Line 1, 2 and 3 are newly added. }
\label{tab:ablation_rebuttal}
\end{table}
